SETGAN: Scale and Energy Trade-off GANs for Image Applications on Mobile Platforms

We consider the task of photo-realistic unconditional image generation (generate high quality, diverse samples that carry the same visual content as the image) on mobile platforms using Generative Adversarial Networks (GANs). In this paper, we propose a novel approach to trade-off image generation accuracy of a GAN for the energy consumed (compute) at run-time called Scale-Energy Tradeoff GAN (SETGAN). GANs usually take a long time to train and consume a huge memory hence making it difficult to run on edge devices. The key idea behind SETGAN for an image generation task is for a given input image, we train a GAN on a remote server and use the trained model on edge devices. We use SinGAN, a single image unconditional generative model, that contains a pyramid of fully convolutional GANs, each responsible for learning the patch distribution at a different scale of the image. During the training process, we determine the optimal number of scales for a given input image and the energy constraint from the target edge device. Results show that with SETGAN's unique client-server-based architecture, we were able to achieve a 56% gain in energy for a loss of 3% to 12% SSIM accuracy. Also, with the parallel multi-scale training, we obtain around 4x gain in training time on the server.

==> files/07_references_shortened.tex <==
@inproceedings{p2m6,
  author    = {Christopher Bongsoo Choy and
               Danfei Xu and
               JunYoung Gwak and
               Kevin Chen and
               Silvio Savarese},
  title     = {3D-R2N2: {A} Unified Approach for Single and Multi-view 3D Object
               Reconstruction},
  booktitle = {Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam,
               The Netherlands, October 11-14, 2016, Proceedings, Part {VIII}},
  pages     = {628--644},
  year      = {2016},
  crossref  = {DBLP:conf/eccv/2016-8},
  url       = {https://doi.org/10.1007/978-3-319-46484-8\_38},
  doi       = {10.1007/978-3-319-46484-8\_38},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/ChoyXGCS16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{p2m13,
  author    = {Kaiming He et. al},
  title     = {Deep Residual Learning for Image Recognition},
  booktitle = {{IEEE CVPR}},
  pages     = {770--778},
  year      = {2016},
  crossref  = {DBLP:conf/cvpr/2016},
  doi       = {10.1109/CVPR.2016.90},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/HeZRS16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{b3,
  author    = {Michael M. Bronstein and
               Joan Bruna and
               Yann LeCun and
               Arthur Szlam and
               Pierre Vandergheynst},
  title     = {Geometric Deep Learning: Going beyond Euclidean data},
  journal   = {{IEEE} Signal Process. Mag.},
  volume    = {34},
  number    = {4},
  pages     = {18--42},
  year      = {2017},
  url       = {https://doi.org/10.1109/MSP.2017.2693418},
  doi       = {10.1109/MSP.2017.2693418},
  timestamp = {Wed, 26 Jul 2017 18:02:24 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/spm/BronsteinBLSV17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{b4,
  author    = {Micha{\"{e}}l Defferrard and
               Xavier Bresson and
               Pierre Vandergheynst},
  title     = {Convolutional Neural Networks on Graphs with Fast Localized Spectral
               Filtering},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {3837--3845},
  year      = {2016},
  crossref  = {DBLP:conf/nips/2016},
  url       = {http://papers.nips.cc/paper/6081-convolutional-neural-networks-on-graphs-with-fast-localized-spectral-filtering},
  timestamp = {Fri, 03 Mar 2017 14:59:41 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/nips/DefferrardBV16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{b5,
  author    = {Thomas N. Kipf and
               Max Welling},
  title     = {Semi-Supervised Classification with Graph Convolutional Networks},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  year      = {2017},
  crossref  = {DBLP:conf/iclr/2017},
  url       = {https://openreview.net/forum?id=SJU4ayYgl},
  timestamp = {Thu, 25 Jul 2019 14:25:55 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/KipfW17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{p2m,
  author    = {Nanyang Wang and
               Yinda Zhang and
               Zhuwen Li and
               Yanwei Fu and
               Wei Liu and
               Yu{-}Gang Jiang},
  title     = {Pixel2Mesh: Generating 3D Mesh Models from Single {RGB} Images},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XI}},
  pages     = {55--71},
  year      = {2018},
  crossref  = {DBLP:conf/eccv/2018-11},
  url       = {https://doi.org/10.1007/978-3-030-01252-6\_4},
  doi       = {10.1007/978-3-030-01252-6\_4},
  timestamp = {Thu, 12 Sep 2019 15:28:49 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/WangZLFLJ18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{p2m26,
 author = {Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
 title = {The Graph Neural Network Model},
 journal = {Trans. Neur. Netw.},
 issue_date = {January 2009},
 volume = {20},
 number = {1},
 month = jan,
 year = {2009},
 issn = {1045-9227},
 pages = {61--80},
 numpages = {20},
 url = {http://dx.doi.org/10.1109/TNN.2008.2005605},
 doi = {10.1109/TNN.2008.2005605},
 acmid = {1657482},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {Graphical domains, graph neural networks (GNNs), graph processing, graphical domains, recursive neural networks},
} 


@inproceedings{p2m24,
  author    = {Jhony K. Pontes and
               Chen Kong and
               Sridha Sridharan and
               Simon Lucey and
               Anders P. Eriksson and
               Clinton Fookes},
  title     = {Image2Mesh: {A} Learning Framework for Single Image 3D Reconstruction},
  booktitle = {Computer Vision - {ACCV} 2018 - 14th Asian Conference on Computer
               Vision, Perth, Australia, December 2-6, 2018, Revised Selected Papers,
               Part {I}},
  pages     = {365--381},
  year      = {2018},
  crossref  = {DBLP:conf/accv/2018-1},
  url       = {https://doi.org/10.1007/978-3-030-20887-5\_23},
  doi       = {10.1007/978-3-030-20887-5\_23},
  timestamp = {Thu, 19 Sep 2019 14:00:20 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/accv/PontesKSLEF18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{p2m17,
  author    = {Hiroharu Kato and
               Yoshitaka Ushiku and
               Tatsuya Harada},
  title     = {Neural 3D Mesh Renderer},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {3907--3916},
  year      = {2018},
  crossref  = {DBLP:conf/cvpr/2018},
%   url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Kato\_Neural\_3D\_Mesh\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00411},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/KatoUH18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{p2m9,
  author    = {Haoqiang Fan and
               Hao Su and
               Leonidas J. Guibas},
  title     = {A Point Set Generation Network for 3D Object Reconstruction from a
               Single Image},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {2463--2471},
  year      = {2017},
  crossref  = {DBLP:conf/cvpr/2017},
  url       = {https://doi.org/10.1109/CVPR.2017.264},
  doi       = {10.1109/CVPR.2017.264},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/FanSG17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{p2m11,
  author    = {Rohit Girdhar and
               David F. Fouhey and
               Mikel Rodriguez and
               Abhinav Gupta},
  title     = {Learning a Predictable and Generative Vector Representation for Objects},
  booktitle = {Computer Vision - {ECCV} 2016 - 14th European Conference, Amsterdam,
               The Netherlands, October 11-14, 2016, Proceedings, Part {VI}},
  pages     = {484--499},
  year      = {2016},
  crossref  = {DBLP:conf/eccv/2016-6},
  url       = {https://doi.org/10.1007/978-3-319-46466-4\_29},
  doi       = {10.1007/978-3-319-46466-4\_29},
  timestamp = {Wed, 25 Sep 2019 18:11:13 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/GirdharFRG16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{p2m30,
  author    = {Maxim Tatarchenko and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {Octree Generating Networks: Efficient Convolutional Architectures
               for High-resolution 3D Outputs},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {2107--2115},
  year      = {2017},
  crossref  = {DBLP:conf/iccv/2017},
  url       = {https://doi.org/10.1109/ICCV.2017.230},
  doi       = {10.1109/ICCV.2017.230},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iccv/TatarchenkoDB17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DenseConnectedNet,
  author    = {Gao Huang and
               Zhuang Liu and
               Kilian Q. Weinberger},
  title     = {Densely Connected Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1608.06993},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.06993},
  archivePrefix = {arXiv},
  eprint    = {1608.06993},
  timestamp = {Mon, 10 Sep 2018 15:49:32 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HuangLW16a},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{shapenet,
  author    = {Angel X. Chang and et. al},
  title     = {ShapeNet: An Information-Rich 3D Model Repository},
  journal   = {CoRR},
  volume    = {abs/1512.03012},
  year      = {2015},
%   url       = {http://arxiv.org/abs/1512.03012},
  archivePrefix = {arXiv},
  eprint    = {1512.03012},
  timestamp = {Mon, 13 Aug 2018 16:47:39 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/ChangFGHHLSSSSX15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{ResNetDeep,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Deep Residual Learning for Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1512.03385},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03385},
  archivePrefix = {arXiv},
  eprint    = {1512.03385},
  timestamp = {Mon, 13 Aug 2018 16:46:56 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HeZRS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@misc{odroidboard,
  author       = {ODROIOD-XU4},
  howpublished = {\url{https://wiki.odroid.com/odroid-xu4/hardware/hardware}},
note = {Online; Accessed 29 March 2018},
year={2017}
}

@article{Eyeriss,
  author    = {Yu-Hsin Chen and Joel Emer and Vivienne Sze},
  title     = {Using Dataflow to Optimize Energy Efficiency of Deep Neural Network
               Accelerators},
  journal   = {{IEEE} Micro},
  year      = {2017}
}
@inproceedings{DaDianNao,
 author = {Yunji Chen and others},
 title = {DaDianNao: A Machine-Learning Supercomputer},
 booktitle = {Proceedings of MICRO},
 year = {2014},
 pages = {609--622}
} 

@article{TETRIS,
 author = {Mingyu Gao and others},
 title = {TETRIS: Scalable and Efficient Neural Network Acceleration with 3D Memory},
 journal = {SIGARCH Computer Architecture News},
  year = {2017}}

@ARTICLE{Survey_v.Sze, 
author={Vivienne Sze and
               others}, 
journal={Proceedings of the IEEE}, 
title={Efficient Processing of Deep Neural Networks: A Tutorial and Survey}, 
year={2017}, 
volume={105}, 
number={12}, 
% pages={2295-2329}
}

@article{DBLP:journals/corr/ZhouYGXC17,
  author    = {Aojun Zhou and
               Anbang Yao and
               Yiwen Guo and
               Lin Xu and
               Yurong Chen},
  title     = {Incremental Network Quantization: Towards Lossless CNNs with Low-Precision
               Weights},
  year      = {2017},
  Journal = {arXiv:1702.03044},
  archivePrefix = {arXiv},
  eprint    = {1702.03044}
}

@article{DBLP:journals/corr/HanPTD15,
  author    = {Song Han and
               others},
  title     = {Learning both Weights and Connections for Efficient Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1506.02626},
  year      = {2015},
  archivePrefix = {arXiv},
  eprint    = {1506.02626},
  timestamp = {Wed, 07 Jun 2017 14:40:54 +0200},
}

@INPROCEEDINGS{FPweights, 
author={Yufei Ma and others}, 
booktitle={Proceedings of FPL}, 
title={Scalable and modularized RTL compilation of Convolutional Neural Networks onto FPGA}, 
year={2016}, 
pages={1-8}
}
@inproceedings{QuantizedDNN,
 author = {Ruizhou Ding and others},
 title = {Quantized Deep Neural Networks for Energy Efficient Hardware-based Inference},
 booktitle = {Proceedings of ASP-DAC},
 year = {2018},
 pages = {1--8},
 numpages = {8},
 acmid = {3201609},
%  publisher = {IEEE Press},
 } 
@article{BinaryDNN,
  author    = {Matthieu Courbariaux and
               Yoshua Bengio},
  title     = {BinaryNet: Training Deep Neural Networks with Weights and Activations
               Constrained to +1 or -1},
  journal   = {CoRR},
  volume    = {abs/1602.02830},
  year      = {2016},
%   url       = {http://arxiv.org/abs/1602.02830},
  archivePrefix = {arXiv},
  eprint    = {1602.02830},
  timestamp = {Mon, 13 Aug 2018 16:46:57 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/CourbariauxB16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@INPROCEEDINGS{Energy-Aware, 
author={Tien{-}Ju Yang and others}, 
booktitle={Proceedings of CVPR}, 
title={Designing Energy-Efficient Convolutional Neural Networks Using Energy-Aware Pruning}, 
year={2017}}

@article{DBLP:journals/corr/LaiSC17,
  author    = {Lai et al.,},
  title     = {Deep Convolutional Neural Network Inference with Floating-point Weights
               and Fixed-point Activations},
  journal   = {CoRR},
  volume    = {abs/1703.03073},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.03073},
  archivePrefix = {arXiv},
  eprint    = {1703.03073},
  timestamp = {Wed, 07 Jun 2017 14:41:48 +0200},
}
@INPROCEEDINGS{CondDeepLearn,
  author    = {Priyadarshini Panda and others},
  title     = {Conditional Deep Learning for energy-efficient and enhanced pattern recognition},
  booktitle   = {Proceeding of DATE},
  year      = {2016}
}
@article{C2F:TCAD2018,
  author    = {Kannappan Jayakodi Nitthilan  and
               others},
  title     = {Trading-Off Accuracy and Energy of Deep Inference on Embedded Systems:
               {A} Co-Design Approach},
  journal   = {{IEEE} TCAD},
  year      = {2018}
  
%   volume    = {37},
%   number    = {11},
%   pages     = {2881--2893},
}

@INPROCEEDINGS{FPweights, 
author={Yufei Ma and Naveen Suda and Yu Cao and Jae-sun Seo and Sarma Vrudhula}, 
booktitle={Proceedings of FPL}, 
title={Scalable and modularized RTL compilation of Convolutional Neural Networks onto FPGA}, 
year={2016}, 
pages={1-8}
}
@article{Xception,
  author    = {Fran{\c{c}}ois Chollet},
  title     = {Xception: Deep Learning with Depthwise Separable Convolutions},
  year      = {2016},
  archivePrefix = {arXiv},
  eprint    = {1610.02357},
}
@INPROCEEDINGS{EIE, 
author={Song Han and others}, 
booktitle={Proceedings of ISCA}, 
title={EIE: Efficient Inference Engine on Compressed Deep Neural Network}, 
year={2016}, 
pages={243-254}}

@INPROCEEDINGS{Cnvlutin, 
author={Patrick Judd and others}, 
booktitle={Proceedings of ISCA}, 
title={Cnvlutin: Ineffectual-Neuron-Free Deep Neural Network Computing}, 
year={2016}, 
pages={1-13}
}

@inproceedings{pesmo,
  title={Predictive entropy search for multi-objective bayesian optimization},
  author={Daniel Hernandez-Lobato and Jose Miguel Hernandez-Lobato and Amar Shah and Ryan P. Adams},
  booktitle={ICML},
  pages={1492--1501},
  year={2016}
}

@inproceedings{ConvFaceDetect,
  author    = {Haoxiang Li and others},
  title     = {A convolutional neural network cascade for face detection},
  booktitle   = {Proceeding of CVPR},
  pages     = {5325-5334},
  year      = {2015}
}

@article{EnergyConstrainedNN,
  author    = {Dimitrios Stamoulis and others},
  title     = {Designing Adaptive Neural Networks for Energy-Constrained Image Classification},
  journal   = {CoRR},
  volume    = {abs/1808.01550},
  year      = {2018},
%   url       = {http://arxiv.org/abs/1808.01550},
  archivePrefix = {arXiv},
  eprint    = {1808.01550},
  timestamp = {Sun, 02 Sep 2018 15:01:56 +0200},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1808-01550},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ICNN-DATE2018,
  author    = {Katayoun Neshatpour and others},
  title     = {ICNN: An Iterative Implementation of Convolutional Neural
Networks to Enable Energy and Computational Complexity
Aware Dynamic Approximation},
  booktitle = {Proceedings of DATE},
  year      = {2018}
}


@inproceedings{PGAN,
title={Progressive Growing of {GAN}s for Improved Quality, Stability, and Variation},
author={Tero Karras and others},
booktitle={ICLR},
year={2018},
% url={https://openreview.net/forum?id=Hk99zCeAb},
}

@inproceedings{singan,
  title={Sin{GAN}: Learning a Generative Model from a Single Natural Image},
  author={Rott Shaham, Tamar and others},
  booktitle={ ICCV, IEEE },
  year={2019}
}

@inproceedings{wp_loss_gan,
  added-at = {2020-03-06T00:00:00.000+0100},
  author = {Gulrajani, Ishaan and others},
  biburl = {https://www.bibsonomy.org/bibtex/2551d042b722228fd8ce03bad7ae3bf5b/dblp},
  booktitle = {NIPS},
  crossref = {conf/nips/2017},
  ee = {http://papers.nips.cc/paper/7159-improved-training-of-wasserstein-gans},
  interhash = {ad4cf89e36acfc121df044f6284b1ed8},
  intrahash = {551d042b722228fd8ce03bad7ae3bf5b},
  keywords = {dblp},
  pages = {5767-5777},
  timestamp = {2020-03-07T11:55:59.000+0100},
  title = {Improved Training of Wasserstein GANs.},
  year = 2017
%   url = {http://dblp.uni-trier.de/db/conf/nips/nips2017.html#GulrajaniAADC17},

  editor = {Guyon, Isabelle and von Luxburg, Ulrike and Bengio, Samy and Wallach, Hanna M. and Fergus, Rob and Vishwanathan, S. V. N. and Garnett, Roman},
  
}

@inproceedings{goodfellow_gan,
  title={Generative Adversarial Nets},
  author={Ian J. Goodfellow and others},
  booktitle={NIPS},
  year={2014}
}

@inproceedings{autoenc_vae,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6114},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaW13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@misc{SP2,
  author       = {SmartPower2},
  howpublished = {\url{https://wiki.odroid.com/accessory/power\_supply\_battery/ smartpower2}},
% urldate = {2017-09-30},
% note = {Online; Accessed 29 March,2018},
% year={2018}
}
@InProceedings{BSD,
  author = {D. Martin and others},
  title = {A Database of Human Segmented Natural Images and its
           Application to Evaluating Segmentation Algorithms and
           Measuring Ecological Statistics},
  booktitle = {IEEE ICCV},
  year = {2001},
  month = {July},
  volume = {2},
  pages = {416--423}
}
@inproceedings{places_dataset,
author = {Zhou, Bolei and others},
title = {Learning Deep Features for Scene Recognition Using Places Database},
year = {2014},
% publisher = {MIT Press},
% address = {Cambridge, MA, USA},
booktitle = {Proceedings on Neural Information Processing Systems},
% pages = {487–495},
numpages = {9},
location = {Montreal, Canada},
series = {NeurIPS’14}
}
@article{mobilenet,
  author    = {Andrew G. Howard and others},
  title     = {MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications},
  journal   = {CoRR},
  volume    = {abs/1704.04861},
  year      = {2017},
%   url       = {http://arxiv.org/abs/1704.04861},
  archivePrefix = {arXiv},
  eprint    = {1704.04861},
  timestamp = {Mon, 13 Aug 2018 16:46:35 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HowardZCKWWAA17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@InProceedings{ref_superresolution,
               author = {Assaf Shocher, Nadav Cohen, Michal Irani},
               title = {"Zero-Shot" Super-Resolution using Deep Internal Learning},
               booktitle = {IEEE CVPR},
               month = {June},
               year = {2018}
              }
@inproceedings{ref_imagemani,
  title={Generative Visual Manipulation on the Natural Image Manifold},
  author={Zhu, Jun-Yan and others},
  booktitle={Proceedings of ECCV},
  year={2016}
}
@inproceedings{img2img,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and and others},
  booktitle={IEEE ICCV},
  year={2017}
}
@InProceedings{ref_paint2img,
author = {Xian, Wenqi  and others},
title = {TextureGAN: Controlling Deep Image Synthesis With Texture Patches},
booktitle = {IEEE CVPR},
month = {June},
year = {2018}
}
@article{texture_syntesis,
author = {Zhou, Yang and others},
title = {Non-Stationary Texture Synthesis by Adversarial Expansion},
year = {2018},
issue_date = {August 2018},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {37},
number = {4},
issn = {0730-0301},
doi = {10.1145/3197517.3201285},
journal = {ACM Trans. Graph.},
month = jul,
articleno = {Article 49},
numpages = {13},
keywords = {non-stationary textures, generative adversarial networks, example-based texture synthesis}
}
@article{texture_syn1,
  author    = {Urs Bergmann and
               Nikolay Jetchev and
               Roland Vollgraf},
  title     = {Learning Texture Manifolds with the Periodic Spatial {GAN}},
  journal   = {CoRR},
  volume    = {abs/1705.06566},
  year      = {2017},
%   url       = {http://arxiv.org/abs/1705.06566},
  archivePrefix = {arXiv},
  eprint    = {1705.06566},
  timestamp = {Mon, 13 Aug 2018 16:49:00 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/BergmannJV17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{texture_syn2,
  title={Texture Synthesis with Spatial Generative Adversarial Networks},
  author={Nikolay Jetchev and Urs Bergmann and Roland Vollgraf},
  journal={ArXiv},
  year={2016},
  volume={abs/1611.08207}
}
@article{pix2pix2016,
  title={Image-to-Image Translation with Conditional Adversarial Networks},
  author={Isola, Phillip and others},
  journal={arxiv},
  year={2016}
}
@inproceedings{vid2vid,
   author    = {Ting-Chun Wang and others},
   title     = {Video-to-Video Synthesis},
   booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},   
   year      = {2018},
}

% IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


==> files/notes.tex <==
[1]
- The reason and explanation for cutting the connection among different-scale generators are not included. The novelty is weak because the design reason is not supported by evidence.
- However, the accuracy result (SSIM) is not compared with the baseline. Besides, the inference time is not compared with the baseline.
-  The paper discusses the selection guidelines according to the application operating scale. Compared with previous works, this work shows a pretty similar result. - Emphasize this
- In Figure 18, the paper shows the examples of random generation with early termination. However, the new figure is too similar to the original picture. The model might be overfitted. More examples should be added to show new structures and object configuration (from SinGAN).




[2]
- In fact, what is placed on the mobile device on the edge is only the inference part. However, the parts that characterize a GAN model is remotely executed. It is far different from the claim. 
- In pg.2 it is mentioned a quick training. Results of SetGAN are quicker than for SinGAN, but still far for being “almost real-time”. Also here a more clear context for the use case would help the reader.
- [xx] in the introduction, it is mentioned the on-line retraining of the network. This lacks of a more clear context.
- [xx] At the end of section II.a it is mentioned that SETGAN is only generative. This again is misleading, since it is only generative on the edge device, but there is the actual training with the generator-discriminator networks on the cloud.
- At the end of pg.3,While for object detection and classification there are clear application contexts and use cases for using them at the edge,  a clear picture of GAN on the mobile device is missing. Without clarifying this point since the beginning of the paper and the proposed approach loses its attractiveness. 
- [xx] Some decisions are not justified. E.g. the use of patches of a single image (Section  IV.a) or parameter of the GAN training (pg.7). Are they derived from other works? How did you reach these decisions? - Mention references
- [xx] At the beginning of page 6, there is a reference to mode #2. The number assigned to each “mode” was missing before that point.
- [xx] The mobile platform that was mentioned in the introduction pops up in the experimental result section, being completely missing during the core part of the work. However, also here is not a central element. 
- [xx] The reason for using EDP as the target metric is unclear. Why EDP and not Energy only? Are you considering a “battery-powered” device or what? Again here there is a completely missing context. The components of the work are there but without the glue to keep them together. 
- [xx] Results on pg9 and pg10 are related to the quality of the output. The authors evaluate them only qualitatively, without any systematic evaluation or comparison with other even simple techniques.




[3]
- [x] However, this client-server design requires frequent data transfer (i.e., image data and weight parameters) between client and server.
On the other hand, a straightforward client-server design is that both the training and inference are performed at the server, and client only sends/receives image data to/from the server.
Regarding data transfer overhead and/or user experience, the benefit of the proposed client-server model against the straightforward design is still unclear to me. It should be clearly demonstrated.
In Table 1, memory utilizations of SinGAN and SETGAN are the same, although SETGAN performs parallel training as shown in Figure 5(b) and 5(c).
So, it seems that memory utilization of SETGAN should be larger than that of SinGAN.
More discussion on this result should be added.


[4]
- [x] It would be useful to include experimental results of the image editing application using other image quality metrics such as no-reference metrics (NIQE, SSEQ, etc.) and even PSNR. Relying on only SSIM is not ideal for characterizing human perception of image quality. 
	- Reference metric. Mention there is not other mechanism and the best among available is SSIM
- [x] In the introduction, I think the paper should include a paragraph about the significance of photo-realistic image generation tasks using GANs.This would provide more context for the paper. Does photo-realistic image generation tasks using GANs consume more energy than other image processing tasks using GANs?
- [x] The paper states that the ODROID-XU4 is popular on current mobile devices, but it might help if the paper explained in more detail why ODROID-XU4 was chosen.
- [x] Fig. 9 shows the effect of training time with the number of scales. The top graph uses the baseline SinGAN model, while the bottom graph uses the optimized SETGAN. For the bottom graph, the training time increases exponentially. For the top graph, the training time also increases exponentially, but slower. What happens if more than 8 scales are used?
- [x] The paper states: "We adapt the SinGAN model [6] since it has a relatively small number of parameters making it an ideal candidate for image editing applications in a client-server architecture." What is the accuracy of GAN models with a larger number of parameters?
- [x] The datasets can be explained more. What kinds of images are in the datasets and how many images are in each dataset?
-------------------------------














































Scale 0, Scle 1 on top of the round boxes, GAN Model (Gi/Di)
Threshold T

All scales trained in parallel

motivate
 Why using Xn upsales is better thant Fn
 
 Multi-scale GANs and Parallel Training

- The drawbacks of existing training (serial) and its impact on image editing applications

- What will parallel training buy you in terms of your overall main goal of applications

- What is the key challenge for parallel training?

- What is your idea to solve that challenge?

- How you train each scale model

(a) Generator

(b) Discriminator

(a) + (b) is a procedure that you use to train GAN model for a particular scale


Why a client server
- Trainign cannot be done on device so that 

Key componet to instantiate
 for a particular application
 Opening paragraph is a base template and each separate application is a specific instantiation of the different application
Number of scales

Summary of experimental section


Memory
Training time
Inference

Existing GAN models are not practical

SETGAN vs PRIOR GANs

Make Table one with just memory and training time. 
Break PGAN and SinGAN are not practical. Then just talk about 

REmove compressed memory and talk about it in some other section talking about client server architecure

Latency for transefering compressed memory latency

Client server - editing where the image has to be sent again and again while in this case 

what 0-3 means in the  memory of individual memoty and not sum

All these number are averaged over the various images


Describe that based on where I inject the image the application changes


Evaluattion of GAN models is still a open topic and mostly evaluated 

Memory and compressed

In first paragraph of introduction, can you add references to those applications

Use a minimal set that will be useful later for the three applications you are studying in this paper

In Paint2Image, what are the input labels

I'm referring to caption of Fig 1

That part is very vague

Can we make it more specific to help the reader

4C (Applications) requires some more clarification, but it can wait

==> notes.tex <==

Early exit idea - exit GAN at a lower level and upsample the other part based on target performance

IS score??? vs battery drain

Using the image complexity to determine the number of layers for doing different image manipulation tasks


SinGAN - decide the number of levels based on image complexity
The model size is small so can be transferred after training
Training happens on remote system and then the small 

The editing process is very compute intensive and so has to be done multiple times. While training is done once and then sent to the mobile. Editing require feedback so done on the mobile

Graphics editing is important

Harmonization, Super Resolution, Image editing, etc

http://www.wisdom.weizmann.ac.il/~vision/ingan/resources/ingan.pdf

https://arxiv.org/pdf/1905.01164.pdf - SinGAN

Remote training and inference on the model

Three applications - namely harmonization, editing, paint2image, random samples

memory consumption of the GAN

Super resolution

SFID based on number of levels

Things to do:
- Find out how SFID changes with levels
- Find out how SFID changes with different images
- Find how SFID changes with image dimensions

- Reduce the computation time by running it with smaller images like 128x128 instead of 256x256 - This would reduce the time to 5 seconds
- Reduce computation by running it with reduced levels
    - It could be 0-N-1
    - or 1 to N - Assuming 1 is the highest dimension this would take more time

- small structures are easily encoded with lesser number of layers


- For each application since editing would be around small regions try estimating the energy and time consumed
    - How does the quality vary with number of levels?
- The three application:
    - in-image painting
    - harmonization
    - paint2image
    - Super resolution

Results:
- How does SFID change with energy for different image types?

Talk about how it is hard to run GANs on mobile platforms. Usual GAN sizes and how it is hard to train one etc







References:
https://github.com/facebookresearch/pytorch_GAN_zoo
https://arxiv.org/pdf/1710.10196.pdf - progressive growing GAN
https://github.com/NVlabs/stylegan
http://openaccess.thecvf.com/content_ICCV_2019/papers/Shaham_SinGAN_Learning_a_Generative_Model_From_a_Single_Natural_Image_ICCV_2019_paper.pdf
https://arxiv.org/pdf/1812.04948.pdf - styleGAN
https://arxiv.org/pdf/1912.04958.pdf - StyleGAN2


file:///Users/kannappanjayakodinitthilan/Downloads/karras2018iclr-paper.pdf
file:///Users/kannappanjayakodinitthilan/Downloads/SingleImageGan_SM.pdf


https://arxiv.org/pdf/1803.04469.pdf - intro
https://arxiv.org/pdf/1511.06434.pdf - UNSUPERVISED REPRESENTATION LEARNING WITH DEEP CONVOLUTIONAL GENERATIVE ADVERSARIAL NETWORKS

